Knowledge-driven Data Construction for Zero-shot Evaluation in Commonsense Question Answering

Recent developments in pre-trained neural language modeling have led to leaps in accuracy on commonsense question-answering benchmarks. However, there is increasing concern that models overfit to specific tasks, without learning to utilize external knowledge or perform general semantic reasoning. In contrast, zero-shot evaluations have shown promise as a more robust measure of a model's general reasoning abilities. In this paper, we propose a novel neuro-symbolic framework for zero-shot question answering across commonsense tasks. Guided by a set of hypotheses, the framework studies how to transform various pre-existing knowledge resources into a form that is most effective for pre-training models. We vary the set of language models, training regimes, knowledge sources, and data generation strategies, and measure their impact across tasks. Extending on prior work, we devise and compare four constrained distractor-sampling strategies. We provide empirical results across five commonsense question-answering tasks with data generated from five external knowledge resources. We show that, while an individual knowledge graph is better suited for specific tasks, a global knowledge graph brings consistent gains across different tasks. In addition, both preserving the structure of the task as well as generating fair and informative questions help language models learn more effectively.

==> Zero-shot Question Answering using Knowledge Bases/1-intro.tex <==
\section{Introduction}
\label{introduction}

Common sense is key to efficient communication in everyday situations, as it enables natural language understanding through contextual reasoning. 
%As McCarthy argued in his seminal work \cite{mccarthy1960programs}, an artificial system has commonsense, {\it if it automatically deduces for itself a sufficiently wide class of immediate consequences of anything it is told and what it already knows}: it follows that machine commonsense can be assessed only by eliciting whether commonsense knowledge and knowledge-based inferences are used by an artificial system in executing a given task.
Machine question answering (QA) benchmarks, like \siqa~\cite{sap-etal-2019-social} and \piqa~\cite{Bisk2020}, are effective {\it behavioral} tests of commonsense reasoning in machines, each focusing on different capabilities. Answering a question in \siqa~might require the knowledge that readers typically prefer heroes over villains in fantasy novels; whereas, in \piqa, the knowledge that metal stools can break windows, because windows are made of glass and metal is a more enduring material than glass. 
Although such tasks had been traditionally difficult for machines, recent developments in pre-trained neural language modeling have led to leaps in accuracy|closing the gap between human and machine performance to single-digit percentage points.\footnote{For example (accessed 4 August, 2020): \url{https://leaderboard.allenai.org/socialiqa/submissions/public}} However, due to increasing concern that large-capacity neural systems are modeling individual datasets, rather than learning how to perform logical reasoning or to utilize external knowledge effectively~\cite{mitra2019exploring}, focus is shifting to alternative training and evaluation strategies.
%\cut{Probes that rephrase a logical prompt show that language models obtain near-random accuracies~\cite{zhou2020can, ribeiro2019red}, and generative evaluation tasks like \commongen~\cite{lin2019commongen} have reported a large gap between human and machine performance. \filip{do we want to say anything about why we don't take the evaluation route?}} 
In particular, \textit{zero-shot evaluation} shows promise as an efficient measure of model generalisability across tasks~\cite{Shwartz2020UnsupervisedCQ,\cut{Banerjee2020SelfsupervisedKT,}li-etal-2020-harvesting}.
%\cut{\filip{Is there a more interesting reason why we do this?}\jf{Not really.}}
Here, models are trained and validated on task $\mathbf{A}$, and tested on a different task $\mathbf{B}$, without access to $\mathbf{B}$'s training data or labels. This leads state-of-the-art models from individual tasks to falter, sometimes  by as much as a 50\% decrease in performance~\cite{Shwartz2020UnsupervisedCQ}. \cut{While \textit{few-shot} evaluation (allowing a few training examples from $\mathbf{B}$) can help, the gaps to the fully-supervised training and human-level performance remain large. }

Repositories of commonsense knowledge, like \conceptnet~\cite{10.5555/3298023.3298212} and \atomic~\cite{DBLP:conf/aaai/SapBABLRRSC19}, can be beneficial for commonsense QA, especially when little or no training data is available.
%
%One approach to closing this gap 
\cut{\km{this gap refers to the gap between zero-shot and human, but the following papers are not addressing this issue in particular}}
%, is the incorporation of external commonsense knowledge repositories.
Enriching the training data with \conceptnet~and \atomic~has been shown~\cite{ma-etal-2019-towards,mitra2019exploring} to improve accuracy on datasets \textit{derived} from these graphs: \csqa~\cite{talmor-etal-2019-commonsenseqa} and \siqa. 
%\citet{ma-etal-2019-towards} show improvements on \csqa~\cite{talmor-etal-2019-commonsenseqa} when using knowledge extracted from \conceptnet~\cite{10.5555/3298023.3298212}, and \citet{mitra2019exploring} find  \atomic~\cite{DBLP:conf/aaai/SapBABLRRSC19} aids accuracy on \siqa~\cite{sap-etal-2019-social}. 
%However, in these cases the evaluation dataset was originally \textit{derived} from the corresponding knowledge resource; and that the benefit of the external knowledge was, therefore, limited to cases where the questions and the knowledge types are well-aligned.
%Including knowledge from \textit{additional} resources does not neccessarily help, as it can lead to noisy or contradicting training samples which harm model performance~\cite{ma-etal-2019-towards}. 
Knowledge bases (KBs) can be used to generate question-answer pairs and distractors automatically, in order to test a model's reasoning ability~\cite{petroni2019language,richardson2019does} or provide additional supervision~\cite{ye2019align,Yang2020GDAUGGD}. 
\cut{\cut{possible solution to these issues\cut{\km{maybe we want to clarify what these issues refer?}}; this is typically seen as a}way of making a given contextual representation more complete \cite{rao-daume-iii-2019-answer}, providing additional supervision \cite{klein2019learning, dhingra-etal-2018-simple}, or of generating tests for models' reading comprehension~\cite{du-etal-2017-learning}. Refinement techniques such as adversarial filtering~\cite{bras2020adversarial} may further improve their quality, by using embedding similarity in order to automatically distill informative questions for a language model. \cut{\km{this sentence seems isolated here}}}
While KBs have been shown to help in a zero-shot transfer setting recently~\cite{Banerjee2020SelfsupervisedKT}, no comprehensive study exists on the relation between various knowledge, its usage method, and neural models for zero-shot transfer across commonsense tasks. Moreover, while adversarial filtering techniques~\cite{bras2020adversarial} improve the quality of a manually created question set, their impact on automatically generated questions from a variety of KBs has not been investigated yet.

%However, few have focused on non-extractive commonsense question-answering as the downstream task: other approaches do not sample strong negative examples as distractor answer-options, as would be required in multiple-choice QA settings. We observe degraded performance of conventional adversarial filtering techniques, when applied to our auxiliary QA data, resulting in bad distractor answer options and unfair (or trivial) questions overall. Furthermore, we observe that the background context used by previous approaches for generating these auxiliary QA pairs is often quite limited|thereby restricting the set of tasks that the resultant pre-trained models can be applied to, despite their intention of achieving high performance under zero-shot and few-shot inference conditions. Finally, few attempts are made to match the \textit{structure} of the generated context with that of the downstream tasks under consideration, thus reducing ease of transfer. 

%\cut{Previous works \cite{missing_citation} show the benefit of prioritizing task-specific exemplars as training samples, as it encourages the language model to understand the \textit{structure} of the task, agnostic of the surface-level semantics. In other cases, intrinsic structure of the context plays a secondary role to the semantic content that can only be expressed by the type of commonsense that matches the downstream task most closely~\cite{ma-etal-2019-towards}.}

%% In this paper, we provide the best of both worlds, through our data transformation...

%\cut{However, the process of creating, encoding, and systematically presenting these exemplars for language models is far from trivial; in most cases, the added benefit from this process remains nominal. \cite{add,missing,citations} \ao{I'm wondering whether it should be clarified what "exemplar" means here: is it a prototypical statement from a task, a template, ...? Or is "examplar" unambiguous in this context (which means I don't know its specific usage here)?} \filip{Later: make the problems we are addressing very concrete (ideally enumerate)}}

%In addition, previous work\filip{citations} has observed that showing task-like exemplars to the language model helps performance, as it allows the model to understand the structure of the task. However, how to create, encode and present these exemplars to be representative for language models is far from trivial. In a recent paper, \filip{example of a recent competitor}; however, the state-of-the-art performance of these methods is still fairly low.

In this paper, (1) we compile a set of hypotheses and design a novel neuro-symbolic framework that investigates the dependency between knowledge sources, question generation techniques, language model (LM) variants, and tasks. Our framework leverages a wide range of KBs, covering visual, social, and concept-based knowledge, to pre-train LMs for zero-shot evaluation on multiple-choice commonsense QA tasks.
(2) Recognizing that the aspect of question generation is especially understudied, we expand on prior work to devise and test four distractor-sampling strategies for effective question generation.\cut{ for non-extractive commonsense QA tasks.}  %Additionally, we show that the naive inclusion of adversarial filtering may be counter-productive.% without careful negative distractor sampling.
We analyze their impact on model performance across tasks, conditioned on model class and (pre-)training regime, and show that generating questions that are simultaneously fair and informative is difficult but beneficial for LM pre-training.
(3) We determine which combination of knowledge graphs (KGs), data construction/training, and architectures is most effective\cut{for transfer to downstream tasks} and can utilize appropriately rich contexts across five tasks.\cut{We provide a systematic evaluation of the effects of on downstream zero-shot model performance for  benchmarks.} We observe that diversifying knowledge generally improves performance, under the condition of it being aligned with the task, and that preserving the structure of the task is desired.
%In summary, this paper's contributions are: (1) We propose a novel neuro-symbolic framework that unifies a wide range of KBs, covering visual, social, and concept-based knowledge. % 
%We transform this unified knowledge graph into a generalizable question-answering dataset, which serves as an auxiliary view of the background context, taking special care to both replicate the structure of downstream tasks as well as preserve the salient type-specific commonsense semantics. This auxiliary data 
\cut{: \anli, \csqa, \piqa, \siqa, and \winogrande.} 
%(2) Building on prior work, we devise four distractor-sampling strategies for QA dataset generation from these KBs and analyze how they affect model performance across tasks, conditioned on model class and (pre-)training regime. We show that preserving the structure of the task, and generating questions that are simultaneously fair and informative is beneficial for language model pretraining.  %Our approach combination of negative sampling and adversarial filtering simplifies learning and improves performance. 
%(3) We provide a systematic evaluation of the effects of knowledge graphs, data construction/training, and architectures on downstream zero-shot model performance for five commonsense benchmarks. We observe that diversifying knowledge generally improves performance, under the condition of it being aligned with the task.
%Throughout our experiments, we systematically vary the source knowledge graph, distractor-sampling method, the language model architecture, and the model pre-training paradigm, in order to investigate each variable's contribution, across the five tasks; we additionally study how the structure of the background context affects these models' inductive capabilities, specifically under zero-shot and few-shot inference conditions. This systematic study enables us to make statements regarding model generalizability across tasks that require different types of commonsense knowledge. Our experiments and ablation studies demonstrate that pre-training language models on our auxiliary QA dataset helps their ability in a zero-shot setting, by clearly outperforming strong baselines. The internals of the language models, the data generation strategy, the choice of background knowledge, and finally the task, all have a measurable effect on the obtained accuracy. 
(4) We make our code and resulting datasets available to the community to facilitate future research in this direction.\footnote{\url{https://github.com/Mayer123/HyKAS-CSKG}} \ \cut{the area of knowledge-driven self-supervision for commonsense QA.}

%In this paper, we propose a novel neuro-symbolic framework that unifies a wide range of knowledge bases, each representing a unique type of common sense, and transforms this structured context into a synthetic question-answer dataset. Through this transformation, we perform adversarial filtering with random distractor-sampling from a constrained set, as a pre-processing step, thereby maintaining task structure while simplifying the learning complexity of the models. Serving as an auxiliary view of these knowledge resources that both replicates the structure of downstream tasks and preserves the salient type-specific commonsense semantics, this synthetic data can then be used for self-supervision, by pre-training language models for downstream application to a wide variety of multiple-choice commonsense QA tasks. Specifically, we generate question-answer pairs from five commonsense knowledge sources: \atomic, \conceptnet, \wordnet, \wikidata, and \visgen; and we make application to the following five multiple-choice commonsense question-answering tasks: \anli, \csqa, \piqa, \siqa, and \winogrande. %
%\cut{We investigate methods to generate artificial QA datasets that can inform language models about the structure and the content of the task. Striving for informativeness and fairness, these methods select answers and distractors based on the graph structure. We pre-train state-of-the-art language models on our synthetic QA sets and evaluate them directly on a diverse set of commonsense reasoning tasks in a zero-shot manner, i.e., without fine-tuning on the task-specific training data.} %The models trained on our synthetic data clearly outperform strong baselines.% by a large margin. 

%In our experiments, we systematically vary the source knowledge graph, distractor sampling method, the language model architecture, and the model pre-training paradigm, in order to investigate each variable's contribution, across the five tasks, and study how the structure of the background context affects these models' inductive capabilities in a zero-shot condition. Our experiments and ablation studies demonstrate that pre-training language models on our auxiliary QA dataset helps their ability in a zero-shot setting, by clearly outperforming strong baselines. The internals of the language models, the data generation strategy, the choice of background knowledge, and finally the task, all have a measurable effect on the obtained accuracy.

%generates a separate view of the  background context in the form of a QA dataset, based on the hypotheses that structured knowledge and task exemplars can enhance neural language modeling performance. 
%We adapt a set of existing knowledge injection models, including HyKAS~\cite{ma-etal-2019-towards}, K-BERT~\cite{liu2020k} and `pure' RoBERTA~\cite{Liu2019RoBERTaAR}, to integrate structured knowledge into a pre-trained language model. 
%We compare two state-of-the-art language models and recently proposed systems on five diverse and large tasks. 

%By doing so, we can mimic the form and the content of various benchmarks. 

%We perform evaluation with different methods and knowledge sources across five benchmarks. %We vary the set of background knowledge sources used to create the auxiliary questions, and we report their impact across the benchmarks. 

%We summarize the contributions of our paper as follows: \begin{enumerate*}
 %   \item We propose a novel and generalizable framework for neuro-symbolic, zero-shot question answering on commonsense tasks. Within the framework, each model is trained once and tested across five different commonsense tasks.
 %   \item We propose a method for pre-training language models, by generating auxiliary question-answer sets from a flexible set of knowledge graphs. We generate questions from five knowledge graphs and sample challenging distractors relying on graph structure. 
 %   \item We use our framework to compare results of different unsupervised models, with and without pre-training with a knowledge graph-based QA. We observe that using KG-based QA consistently yields best performance, and that different knowledge graphs are suitable for different problems.
%    We evaluate the impact of these questions on an array of knowledge injection methods on five commonsense benchmarks. We observe that KG-based QA datasets can inform language models on zero-shot tasks, but this is largely dependent on the alignment between the kind of knowledge captured by these questions and by the graphs.
%    \item In further analysis, we measure the impact of different training regimes and data generation strategies. We observe that marginal ranking~\cite{tamborrino-etal-2020-pre} training yields better performance than language model training, and that combining filters based on the KG structure and on adversarial factors is a viable way to generate QA datasets. The datasets created in this way can help LMs learn more effective, but the success depends on the knowledge types covered by the knowledge graphs. 
    %both informative and fair, as they are most challenging for `vanilla' language models while being easy to solve by humans.
%\end{enumerate*}



==> Zero-shot Question Answering using Knowledge Bases/2-related-work.tex <==
\section{Related Work}

%\filip{proposal: combine and shrink the first two sections}



\subsection{Knowledge Injection}

% The task of commonsense reasoning has attracted a renovated interest over the past two years. It is typically framed as a multiple-choice challenge of selecting one or more correct answers given certain context/premise. Benchmarks~\citep{zellers-etal-2018-swag,zellers-etal-2019-hellaswag,huang-etal-2019-cosmos,zhou-etal-2019-going,Bisk2020} have been developed to evaluate systems on a wide range of common sense skills, such as social or physical understanding. %' ability to tackle various aspects of commonsense the model's progress in this direction , each posing challenges to the models in a different dimension. 

\cut{Commonsense capabilities on a variety of topics (e.g., social or physical understanding) are commonly evaluated by multiple-choice QA benchmarks, like %\texttt{SWAG}~\citep{zellers-etal-2018-swag},
\siqa~%\cite{sap-etal-2019-social},
%\texttt{HellaSwag}~\citep{zellers-etal-2019-hellaswag}, %\texttt{MCTACO}~\citep{zhou-etal-2019-going}, 
%\texttt{Cosmos QA}~\citep{huang-etal-2019-cosmos}, 
and \piqa~%\citep{Bisk2020}.
}
Strong performance on standard multiple-choice QA benchmarks, like \siqa~and \piqa, has been achieved by fine-tuning a task-specific prediction layer, placed atop pre-trained LMs, such as BERT \citep{devlin-etal-2019-bert}, RoBERTa \citep{Liu2019RoBERTaAR}, and GPT \citep{radford2019language}. 
%The performance of these models can be further boosted through techniques such as adversarial training \citep{Zhu2020FreeLB:,pereira-etal-2020-adversarial} and transfer learning \citep{Khashabi2020UnifiedQACF}. 
%\cut{\filip{How about we skip the next two sentences and merge the two paragraphs?} While these models achieve high accuracies on many commonsense tasks, they rely heavily on a large amount of labeled data. On the other hand, we approach these tasks in zero-shot fashion and without fine-tuning on each dataset. \jf{Zero-shot evaluation is not a training paradigm; therefore, the comparison to strong supervision is not fair. Zero-shot evaluation also cannot be a contribution of this paper; at best, it is an assumption or condition.}}%
% \begin{itemize}
%     \item General background on using neural models for commonsense
%     \item Some approaches just rely on using language models (e.g., without any external knowledge resources and/or without any \textit{task-specific} commonsense injection mechanisms)
%     \item MLM pre-training, which may not be best-suited for CS MC QA tasks
% \end{itemize} 
As shown by \citet{ma-etal-2019-towards} and \citet{mitra2019exploring},
combining neural methods with structured background knowledge from \conceptnet, \wordnet~\citep{10.1145/219717.219748}, and \atomic~ works well for commonsense datasets that have been partially derived from these resources, such as \siqa~ and \csqa. Here, the structured knowledge, formalized as lexicalized task-targeted evidence paths, is injected into an LM, either
% , by lexicalizing task-relevant evidence paths from the resource to be encoded  and fed into a neural decision making system. 
\cut{The injection of such structured evidence into a LM can be done with }via an attention mechanism \citep{bauer-etal-2018-commonsense} or through an auxiliary training objective \citep{10.1145/3357384.3358165}. Graph and relation networks can also be used to score answer candidates, by informing the graph structure with data from LMs~\citep{lin-etal-2019-kagnet,10.1007/978-3-030-32233-5_2}. %(FI: I think KagNet (Lin et al., 2019) and MultiGRN (Lin et al., 2020) also fall in the graph category.)  
Finally, complete KGs can be incorporated directly in training by introducing additional modeling objectives, to teach a model about general commonsense regardless of the task at hand~\citep{peters-etal-2019-knowledge,levine-etal-2020-sensebert,Liu2020KBERTEL,zhang-etal-2019-ernie,talmor2020teaching}. This line of work resembles our approach of including background knowledge in a general, task-agnostic way; however, it still relies on the task training data and has generally not been tested in a zero-shot regime.
%(FI: I think the par could be shortened in the beginning; but we should finish by saying how we compare to this work)


%\cut{\jf{I renamed this subsection, from \textit{Zero- and Few-shot Question Answering} to \textit{Generating Commonsense Questions and Answers}. Without discussion of the latter, our overall Related Work section would not be properly configured for comparing our methods with other works that also generate datasets/views/augmentation. Since this ``data transformation'' is the main novelty of the paper, I now feel like we should have an entire subsection in the Related Work section that is dedicated to this dimension. We will need to answer the question(s) of `Why do we need to generate an auxiliary dataset \textit{this} way, and how is our way of doing it better than others?' Self-Talk \cite{Shwartz2020UnsupervisedCQ}, for example, has such a subsection, entitled `Generating Questions and Explanations'. It is possible to re-frame the original content (below, which talked about `Zero- and Few-shot Question Answering') to talk about this instead. In itself, the topic of ``zero-shot/few-shot QA'' is less important, since those are just evaluation paradigms and do not really require motivation beyond what is discussed in the Introduction.} }
%Several approaches have attempted to use knowledge graph in order to train a QA model in a zero-shot fashion, or prompts its accuracy. 

\subsection{Generating Commonsense Questions and Answers}

\citet{richardson2019does} use links in \wordnet~to generate question-answer pairs, %Each question covers one single-hop relation in these resources, and if available, includes an example sentence with the head of the triple. 
then leverage the resulting dataset to evaluate language models. ~\citet{petroni2019language} prompt the skills of language models by sentences instead of questions, generated from sources like \texttt{ConceptNet} and SQuAD~\cite{rajpurkar2016squad}.
Previous works have generated synthetic QA sets to complement existing training data. \cut{model training, albeit mostly in addition to existing training data.} \citet{ye2019align} proposed an `align-mask-select' method to generate questions using \texttt{ConceptNet} and Wikipedia. \citet{kocijan-etal-2019-surprisingly} constructed a large set of pronoun resolution questions using Wikipedia sentences. \citet{Yang2020GDAUGGD} generate QA pair and distractors using generative models. %Unlike our focus on zero-shot evaluation, these efforts use questions to augment the task training data. %, our focus is on zero-shot evaluation. 
%Assuming low availability of training data, the self-training method by \cite{niu2020self} enhances the small set of golden labels with noisy evidence labels, and iteratively uses the pseudo evidence predictions as extra supervision in next iterations. 
%An iterative approach is also used by \citep{li-etal-2020-harvesting}, who use a knowledge graph to generate pre-training data for SQuAD - however, this approach has not been evaluated on commonsense tasks. 
%Another line of work attempt to leverage the generative nature of pretrained language models to fill gaps in tasks,
Regarding zero-shot evaluation, the Self-Talk model of~\cite{Shwartz2020UnsupervisedCQ} generates clarification prompts based on a template prefix, which are leveraged to elicit knowledge from another LM, which is used jointly with the original context and question to score each answer candidate. 
%Most similar to our work, 
Given a task context, one can use COMET~\citep{Bosselut2019DynamicKG}, a generative model trained on commonsense KGs, to generate background knowledge statements, and to compute scores for each answer candidate based on the context, question, and generated knowledge.
\citet{Banerjee2020SelfsupervisedKT} pre-train the LM with three representation learning functions which aim to complete a knowledge triple given two of its elements. These functions jointly compute the distance for each answer candidate. The ambition of this paper is to provide a comprehensive framework for such prior efforts on zero-shot QA with KGs. By covering a wider set of KGs, question generation techniques, and tasks, we can systematically investigate the effect of using different KGs, generation methods, and techniques across tasks.

% our method creates an artificial task based on flexible set of knowledge graphs and construction methods, allowing us to systematically investigate the effect of using different KGs, generation methods, and techniques across tasks.

%Unsupervised methods have been explored in previous works to solve question answering tasks.

%Several papers have also attempted to solve commonsense reasoning tasks in a zero-shot fashion. 
%Given a task context, one can use COMET~\citep{Bosselut2019DynamicKG}, a generative model trained on commonsense knowledge graphs, to generate background knowledge statements, and to compute scores for each answer candidate based on the context, question and generated knowledge.
%To leverage the generative nature of pretrained language models to fill gaps in tasks, the Self-Talk model by~\cite{Shwartz2020UnsupervisedCQ} generates clarification prompts based on a template prefix, which are leveraged to elicit knowledge from another knowledge source (a language model or ConceptNet). The additional knowledge is used jointly with original context and question to score each answer candidate. 
%\cite{shin2020life} shows that automatically generated prompts may elicit more accurate factual knowledge \textcolor{red}{(AO: I removed here and in other parts "factual" or "facts": a fact is an instance of some general knowledge, but the commonsense we talk about in the paper, and assessed in all the tasks we discussed, is not factual)} compared to manual prompts. 
%  Most similar to our work, \cite{Banerjee2020SelfsupervisedKT} pre-train the language model with three objective functions which aim to complete a knowledge triple given two of its elements. These representation learning functions are used jointly to compute the distance for each answer candidate. In contrast to prior work on zero- and few-shot learning with knowledge graphs, our method creates an artificial task to train an option comparison network model. In addition, we systematically investigate the effect of using different knowledge graphs and systems across commonsense tasks.

%pre-train the LM solely based on knowledge graphs. They trained 3 mapping functions to recover the third element in the knowledge triple given the other 2. Then these functions are used jointly to compute the distance for each answer candidate. 
%(FI: we need closure to this par too; how we compare to this work)

==> Zero-shot Question Answering using Knowledge Bases/3-approach.tex <==
\section{Zero-Shot QA Framework}

Given a natural language question $Q$, and $n$ possible answers $A_1, ..., A_n$, the task \cut{of a system (human or machine)} is to select the most probable single answer $A$. We refer to the remaining $n-1$ possible answers: $D_1, ..., D_{n-1}$ as distractors. In a zero-shot QA evaluation mode, the system has no access to the task training or development data. 
We assume a setup where the system is pre-trained once and then applied across different tasks in a zero-shot manner. Our zero-shot evaluation framework addresses this task by variants of pre-training an LM on an artificial QA set, created from KG data. Next, we describe its covered tasks, sources of knowledge, question generation strategies, LM techniques, and training regimes, in turn.\cut{ of our framework.} \cut{We describe each of these dimensions, in turn.}

%In this section, we describe the set of knowledge bases, synthetic data generation strategies, model variants, and tasks covered by our experimental framework.

% \subsection{Commonsense Knowledge Graph (CSKG)}

% We employ the Commonsense Knowledge Graph (CSKG)~\cite{ilievski2020consolidating} in order to generate artificial questions, answers, and distractors. CSKG consolidates seven knowledge sources: ATOMIC, ConceptNet, FrameNet, WordNet, Wikidata, Roget, and Visual Genome, through a set of automatic and manual mappings. Currently, CSKG describes 4.5 million nodes with 17 million edges. It contains an associated sentence and question for its triples, in order to facilitate easier utilization in downstream reasoning tasks.

% For the artificial QA set, we select the knowledge from CSKG in the following way: 1) ...

\subsection{Synthetic QA Generation}
%\filip{Optionally, we could split this to give the KGs their own subsection.}

%\filip{informativeness and difficulty criteria - elaborate}

We generate questions, answers, and distractor options from five KGs: \atomic, \conceptnet, \wordnet, \visgen~\cite{krishna2017visual}, and \wikidata~\cite{vrandevcic2014wikidata}, found in the \CSKG~(\cskg)~\cite{ilievski2020consolidating}. Notably, \texttt{ATOMIC} differs from the other KGs in two ways: 1) its relations have a different focus than those of the other sources; and 2) its node labels are longer and formalized as templates. Due to these considerations, we prepare two sets of QA sets: one based on \texttt{ATOMIC} and one based on the remaining four knowledge sources. Figure \ref{fig:generation} illustrates our question generation pipeline. % The generation of negative samples, however, is identical for both data subsets.

\subsubsection{Data partitions} 
\texttt{ATOMIC} expresses pre- and post-states for events and their participants with nine relations. Its head nodes are events, whereas the tail nodes are either events or attributes. Its nodes have two particularities: 1) irrelevant parts of the node text are replaced with blanks (`\_'); and 2) references to fictional agents are indicated with special tokens (e.g., \textit{PersonX}). We follow the \siqa's \texttt{ATOMIC} train/dev/test splits, to ensure that the facts of the dev and test partitions are excluded in training. % the original ATOMIC train/dev/test split, we follow the same split to create our synthetic dataset.\filip{we don't use the dev/test set - this is fair}

Our second partition, \texttt{CWWV}, covers three other KGs in \cskg~\cut{\km{is this the first mention of CSKG?}}that express commonsense facts between concepts: \conceptnet, \wordnet, and \wikidata. We use them jointly to generate questions, and we enrich them with additional distractors from \visgen. Treating these four sources as a single one is enabled by their \cskg~mapping to a single set of relations, defined by \conceptnet. We focus on 14 semantic relations that are grounded on strong psycholinguistic and pragmatic evidence \cite{murphy2003semantic}, like \texttt{/r/Causes} and \texttt{/r/HasPrerequisite}. Since there is no pre-defined train/dev/test split for \cskg, we randomly sample 5\% of generated questions as development set, while the other 95\% are used for training, to maximize the coverage of the knowledge.  

\begin{figure}[!t]
\includegraphics[scale=0.23]{data_generation.png}
\caption{An illustration of our question generation pipeline.\cut{\filip{we need to explain the example here...}}}
\label{fig:generation}
\end{figure}


\subsubsection{Generating questions and answers}
\cut{\todo{Can we have a nice figure diagram/cartoon that illustrates this process (including the negative samples)?  I'm concerned this bit is crucial but confusing}}
%Given a knowledge triple ($h$, $r$, $t$), 
If a triple ($h$, $r$, $t$) has an associated sentence, we directly employ it for question generation; otherwise, we generate a sentence in a lexicalization step, using a set of pre-defined templates. Next, we generate the question $Q$ by removing the tail of the sentence, and extract this tail as the correct answer, $A$. %For the remaining triples, we generate a sentence , using GPT-2 to choose the lowest perplexity formulation out of a number of predefined templates.  For the lexicalized sentences, we remove the tail $t$ and use it as the correct answer, $A$. 
Here, we ensure that there is no token overlap between the head and the correct answer. For \texttt{ATOMIC}, we: 1) compare the keyword tokens instead of all tokens, in order to avoid stopwords; and 2) the agent templates (e.g., `PersonX') are replaced with randomly sampled gender-neutral names from a pre-defined set.
For \texttt{CWWV}, we filter out questions where either the head or the tail are not common concepts or they are named entities. We use corpus frequency as a proxy for commonness,\footnote{\url{https://pypi.org/project/wordfreq/} (Accessed 9 Sept. 2020)} while named entities are filtered by removing all concepts whose labels start with a capital letter. 
%For instance, given a triple \textit{(PersonX takes the fifth, xWant, withhold information)} in ATOMIC, this step yields the question \textit{Robin takes the fifth. As a result, Robin wanted to} with a correct answer \textit{withhold information}.

%we first convert it into a sentence by using a relation-based template.\footnote{For a small set of triples, we make use of the associated human-generated sentences instead of lexicalization.} For each relation, we pre-define a set of templates and 

% For example, we convert \textit{(PersonX plays a \_\_\_ in the war, xIntent, to participate)} to  \textit{PersonX plays a \_\_\_ in the war because PersonX wanted to participate}. We pre-define one template for every ATOMIC relation as done in COMET. 
% %Next, we fill the aforementioned blanks in the sentence using the RoBERTa pre-trained model, by masking the blanks and directly using RoBERTa to predict the missing word. 
% The adapted head node and relation is used as a question, $Q$, while the adapted tail is used as the correct answer, $A$. 
% We ensure that there is no keyword token overlap between the head and the correct answer, as the overlap may make the question easy to solve.
% %To obtain the question, $Q$, we use templates to convert the ATOMIC relation into a question. An example ($C$, $Q$, $A$) is (PersonX plays a role in the war, Why did PersonX do this?, to participate).
% %Next, we separate out the original head and tail of the node, which will be used later as the context and correct answer respectively. 
% %Then we define another set of templates to convert every ATOMIC relations into a question, which would yield a (C, Q, A) triple, i.e. (PersonX plays a role in the war, Why did PersonX do this?, to participate). 




\begin{table}[t]
  \begin{center}
    \small{
    \caption{Generated questions from \atomic~ (top) and \texttt{CWWV} (bottom). (*) denotes the correct answer.}
    \label{tab:example}
    \begin{tabular}{@{}l@{}} 
     \toprule
      Question: Robin takes the fifth. As a result, Robin wanted to\\
      A1: go to the cinema. \\
      A2: withhold information. (*)\\
      A3: hear what they think. \\
    \midrule
      Question: losing weight is for \\
      A1: being healthier. (*) \\
      A2: embedded software. \\
      A3: buying things in store. \\
      %Question: 0 degrees farenheit is \\
      %A1: very cold. (*) \\
      %A2: important in italian culture. \\
      %A3: normal during day. \\
    \bottomrule
    \end{tabular}
    }
  \end{center}
\end{table}
\subsubsection{Generating negative samples (distractors)}

We seek to generate distractor options that satisfy two criteria: \textit{informativeness} and \textit{fairness}. Namely, a good distractor has semantic relatedness with the context (informative), while being relatively easy to discriminate from the correct answer (fair).
We create the pool of distractors $D$ for every sample as follows:
\begin{enumerate*}
    \item The distractor candidates are the tails of knowledge triples ($h'$, $r'$, $t'$) with the same relation $r' = r$, randomly sampled from the KGs. This would ensure that the distractors can fill the same semantic role as the correct answer. 
    \item The head $h'$ of the sampled triples does not have non-stop word overlap with $h$. %We compute these overlaps based on the keywords as given by ATOMIC
    \item The distractor tail $t'$ is not part of the correct answer set, i.e., there exist no triples, ($h$, $r$, $t'$)
    %\item $t'$ is not a substring of $t$ or the other way around
    %\item we perform adversarial filtering~\cite{}, by computing sentence embeddings for each distractor and ensure that its similarity to the answer is as high as possible, yet lower than a preset threshold.
\end{enumerate*}. 
%In addition,  
\cut{These rules would help ensure that the distractors are semantically similar to the answer, while not being correct answers, thus making them simultaneously challenging and fair.}
Considering the example in Figure \ref{fig:generation}, the triple \textit{(gaining weight, CausesDesire, change appearance)} will be filtered out by rule (1), \textit{(losing weight, UsedFor, feeling better)} will be ruled out by both (2) and (3), and \textit{(relaxing, UsedFor, feeling better)} will be ruled out by (3). Here, we replace any references to fictional \texttt{ATOMIC} agents in the distractors with the same names used in the question. We then randomly select two distractors ($D_1$, $D_2$) from $D$. We refer to this distractor pooling strategy as \textit{random}, and propose three alternative strategies in the next Section. % \textit{Distractor sampling}. 

Example questions with each partition are shown in Table~\ref{tab:example}. For \atomic, this procedure generates 535K QA pairs for training and 60K for development. For \texttt{CWWV}, the training set contains 157K and the dev set has 8K QA pairs.

%Finally, we randomly sample a set of gender-neutral names from a pre-defined set to replace all agent references in $Q$, $A$, $D_1$ and $D_2$. %E.g. PersonX $->$ Bob, PersonY $->$ Alex. 
 
%We split ATOMIC into a train and a dev set, after which 
%e do not create QA pairs for triples whose tail has overlap with keywords in the head, as the overlap may make the question trivially easy to solve.

% If the triple has an associated sentence, then we generate $Q$ by masking the tail of the sentence, and extract this tail as the correct answer, $A$. For the remaining triples, we generate a sentence in a lexicalization step, using GPT2 to choose the lowest perplexity formulation out of a number of predefined templates. For the lexicalized sentences, we mask the tail and use it as the correct answer, $A$. Here, we also ensure that there is no token overlap between the head and the correct answer.

%of these relations, we either: 1) generate questions by using templates; 2) use existing sentence or generate one in a lexicalization step, and mask the answer word (corresponding to the tail of the triple). For instance, given the triple ``0 degrees fahrenheit - IsA - very cold'', we use the OMCS sentence as a starting point (or generate one if this is missing), leaving us with: ``[[0 degrees fahrenheit]] is [[very cold]].''. Next, we normalize the head and mask the tail as follows:  ``0 degrees fahrenheit is [MASK].'' At this point our question-answer pair is ready.

%To generate distractors, given a question triple ($h$, $r$, $t$), we gather tails from triples ($h',r',t'$), for which $r' = r$ and $h'\neq h$. Essentially, this provides us with other objects that fulfill the role of a tail for the same relation, but are not valid for the same head. We exclude distractors which have a token overlap with the correct answer. We implement this procedure by collecting a set of tails $T$ for each head-relation pair, and then we sample two distractors per question from $T$. In addition, we filter out questions where either the head or the tail are not common concepts or they are named entities. We use corpus frequency as a proxy for commonness,\footnote{\url{https://pypi.org/project/wordfreq/}} while named entities are filtered by removing all cases which contain a capital letter. An example entry is shown in Table~\ref{tab:example} (bottom). %Since there is no pre-defined train/dev/test split for CSKG, we randomly sample 5\% of generated questions as development set and used the other 95\% for training.  


% \begin{table}
%   \begin{center}
%     \caption{Example: a generated example from CSKG (w/o ATOMIC), where the asterisk (*) denotes the correct answer}
%     \label{tab:example_cskg}
%     \begin{tabular}{l} 
%      \hline
%       Question: 0 degress farenheit is [MASK] \\
%       A1: very cold (*) \\
%       A2: important in italian culture \\
%       A3: normal during day \\
%     \hline
%     \end{tabular}
%   \end{center}
% \end{table}




%follow the following graph patterns: a) labels of tail nodes that share the same head, but not the relation; b) head node labels that share the same tail, but not the relation. Next, we normalize the set of distractors by selecting a single distractor per relation, when there are multiple. If the remaining number of distractors for a question is greater than the number of distractors needed for a single question, we generate multiple questions. Questions that have insufficient distractors are completed by randomly sampling a distractor based on the question relation.

\subsection{Distractor Sampling}
Existing data generation procedures are likely to introduce annotation artifacts in datasets \cite{zellers-etal-2019-hellaswag,sakaguchi2019winogrande}. Models may exploit these artifacts to achieve spuriously strong performance during training, at the expense of degradation in robustness.
To generate more challenging QA pairs from KGs and to alleviate potential biases in our synthetic sets, we test two other distractor sampling strategies in addition to the \textit{random} strategy: 1) we select distractors that are as similar as possible to the answer, while being under a certain threshold (\textit{adv-answer}); and 2) we select distractors that are as similar as possible to the question, while being under a certain threshold (\textit{adv-question}). Here we define similarity of two nodes to be their proximity in the embedding space, measured by cosine similarity. The intuition is that, by generating more challenging QA pairs for the models, we could achieve better generalization across tasks. We use the RoBERTa sentence embedding model~\cite{reimers-2020-multilingual-sentence-bert} to compute embeddings for all KG nodes. For these two strategies, we set an upper bound on the similarity score to avoid unfair distractors, i.e., paraphrases of the correct answer. Based on manual observations, we set their distractor similarity upper bound to be 0.6 for \texttt{CWWV} and 0.4 for \texttt{ATOMIC}.

\subsubsection{Sample filtering}
Besides these distractor sampling strategies, we test another condition (3), where we select the distractors randomly, but only keep the questions whose distractors are sufficiently challenging at training time (\textit{adv-filter}). The intuition is that QA pairs generated using the aforementioned methods might still be too easy for the models, thus we would like to only keep the most challenging subset to train our models. We employ the AFLite algorithm \cite{sakaguchi2019winogrande} for our purpose. Given a \textit{train} and \textit{dev} split of our synthetic QA set, we use 5\% of the \textit{train} set to finetune a RoBERTa model with a classification head (4\% training, 1\% validation). These 5\% are discarded from \textit{train} after this step. We then compute the fixed embeddings for the remaining 95\% of \textit{train} and the entire \textit{dev}, denoted as \textit{Trn} and \textit{Dev}. Next, we feed \textit{Trn} and \textit{Dev} along with their labels to the AFLite algorithm, which iteratively filters out easy examples using an ensemble of linear classifiers. Finally, we retain (101K training, 11K dev) samples for \texttt{ATOMIC} and (29K training, 1.5K dev) samples for \texttt{CWWV} subset. The details of AFLite can be found in the appendix.

\cut{we partition the remaining 95\% of \textit{train} into \textit{train-sub} and \textit{train-dev} set, and train a linear classifier taking the computed embeddings as the input on the \textit{train-sub}. (d) We make prediction on \textit{train-dev} and \textit{dev} sets. (e) We repeat step (c) and (d) for K times and train a new classifier on a different partition each time. (f) We filter out examples that has prediction accuracy greater than $\tau$. (g) While the remaining size of \textit{train} is larger than \textit{Target} or the newly discarded sample is greater than \textit{k}, repeat step (e) and (f).}\cut{\filip{the algorithmic steps are a bit hard to follow. Perhaps we should turn this into an Algorithm with pseudo code.}  \filip{i propose we move parameter settings to implementation}}





\subsection{Language Models}
%Following previous work, we establish several baselines using pre-trained language models. Here 
We consider 2 types of language models: auto-regressive language models and masked language models (MLM). Specifically, we use GPT-2 and RoBERTa to select the best answer candidate. Given a context $C$, a question $Q$, and a list of answer options ($A_1, A_2 ... $), we concatenate $C$ and $Q$ with each answer option to build input sequences ($T_1, T_2 ... $). We also use templates to convert a sequence $T$ into a natural language sentence following \cite{Shwartz2020UnsupervisedCQ}. 
For example, we transform the sequence: \textit{[$C$] What will X want to do next? [$A_i$]}  into: \textit{[$C$], as a result, X want to [$A_i$]}. The score $S$ for the resulting sequence using an auto-regressive LM is computed as follows:
\begin{equation}
    \mathrm{S_{LM}}\left(T \right)=-\frac{1}{n} \sum_{i=1}^{n} \log P\left(t_{i} \mid t_{1} \ldots t_{i-1}\right)
\end{equation}
where $n$ is the number of tokens in the sequence and $P$ is the conditional probability provided by the LM. To evaluate MLMs, we mask out one token at a time and compute its loss~\cite{Zhou2020EvaluatingCI}. We repeat this process for every token in the sequence. The final MLM score is:
\begin{equation}
    \mathrm{S_{MLM}}\left(T \right)=-\frac{1}{n} \sum_{i=1}^{n} \log P\left(t_{i} \mid \ldots t_{i-1},  t_{t+1} \ldots \right)
\end{equation}
The predicted option is the one with the lowest score. 

  

\subsubsection{LM Finetuning}
In the typical model architecture for finetuning LM for multiple-choice tasks, a linear layer is added on top of the LM encoder to predict the answer. The model inputs are separated by a model-specific delimiter. However, as this architecture introduces randomly initialized parameters, it may not be able to fully utilize the pre-trained weights~\cite{tamborrino-etal-2020-pre}. 
Instead, we re-use the GPT-2 and RoBERTa with LM head for finetuning.
%We adopt the same~\filip{same as Tamborino, or same as eq2?} model architecture as LM baselines, i.e. encoder with a LM head. 
%We keep the same input converting templates and scoring functions as in the original LM baseline.
By keeping the model intact, we can reuse the same converting templates and scoring functions.
To train the model, given the scores computed for each answer candidate $S_1, S_2, ... S_m$, we use the marginal ranking (MR) loss defined as:
\begin{equation}
    \mathcal{L}=\frac{1}{m} \sum_{i=1 \atop i \neq y}^{m} \max \left(0, \eta-S_{y}+S_{i}\right)
\end{equation}
Here, $\eta$ represents the margin and $y$ is the index of the correct answer. For a MLM model, the computation cost for the scoring function scales quadratically with the input length. To make the training more efficient, we only mask out non-stop tokens in the head and tail nodes. 
% We adopt the typical model architecture for finetuning LM for multiple-choice tasks. Specifically, given C, Q and ($a_1, a_2 ... $), C and Q is concatenated with each $a$, separated by model-specific deliminator tokens. Then each sequence is fed to the LM encoder separately and the final layer's output of [CLS] token is chosen to be the sequence representation. A linear layer is added on top of LM encoder to predict the answer, taking all answer candidate's sequence representation as inputs.  

% We train the GPT-2 large and RoBERTa large models on the synthetic training set for three epochs. The checkpoint that yields the best performance on our synthetic dev set is saved and used for evaluation in our experiments.

% \subsubsection{HyKAS} We adopt the HyKAS model proposed by \cite{ma-etal-2019-towards}, which consists a language model encoder and the Option Comparison Network (OCN) \cite{Ran2019OptionCN}. It is worth noting that we did not use the knowledge inject cell of the HyKAS model as our synthetic dataset do not have extra knowledge triples. The original OCN expects a fixed number of answer candidates, since the tasks we evaluate on contain different number of options, we modified the OCN to make it more flexible. Specifically, we 
% How do we explain this? 

\subsubsection{Training Regimes}
In order to disentangle the contribution of the KGs from the structure of the QA pairs, we consider different training methods for augmentation of language models with KGs. Specifically, we compare marginal ranking (MR) training with masked language modeling (MLM) training. For MLM, we directly concatenate the question and the correct answer in our synthetic QA set and then train RoBERTa on the these sentences using the MLM objective.\cut{\filip{not sure why is this a separate section}}



\begin{table*}[t]
  \begin{center}
    \caption{
    Zero-shot evaluation results with different combinations of models and knowledge sources, across five commonsense tasks. \texttt{CSKG} represent the combination of \texttt{ATOMIC} and \texttt{CWWV}. We run our experiments three times with different seeds and report average accuracy with 95\% confidence interval. SMLM (*) used OMCS for CSQA, ROCStories \cite{mostafazadeh-etal-2016-corpus} for aNLI and ATOMIC for SIQA as knowledge resources. 
    \cut{Model results under zero-shot inference conditions. \jf{Many different dimensions are captured in this table, and we should carefully describe the distinctions: pre-training vs. not pre-training, ATOMIC vs. CSKG, unsupervised vs. supervised, MLM vs. `new'. We need to emphasise that all the methods that are currently in the `unsupervised (pre-trained)' section (that specifically use \atomic~or \texttt{CSKG}) are ``ours". We should consider adding results for pre-training on a competing QA-generation approach.}. \jf{Explain ``Majority", here in the caption.}. The asterisk (*) denotes the test set accuracy.}
    }
    \label{tab:zero-shot}
    \begin{tabular}{@{}l@{\hspace{5pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{}} 
     \toprule
    \bf Model & \bf KG &  \bf aNLI  & \bf CSQA & \bf PIQA & \bf SIQA & \bf WG \\
      \midrule
       Majority & - & 50.8 & 20.9 & 50.5 & 33.6 & 50.4 \\
      GPT2-L & - & 56.5  & 41.4 & 68.9 & 44.6 & 53.2 \\
      RoBERTa-L & - & 65.5  & 45.0 &  67.6 & 47.3 & 57.5 \\
      Self-talk \hfill \cite{Shwartz2020UnsupervisedCQ} & - & -  & 32.4 & 70.2 & 46.2 & 54.7\\
      COMET-DynaGen \hfill \cite{Bosselut2019DynamicKG} & \texttt{ATOMIC} & - & - & -  & 50.1 & - \\
      SMLM     \hfill \cite{Banerjee2020SelfsupervisedKT} & \texttt{*} & 65.3 & 38.8 & - & 48.5 & - \\
      \midrule
      GPT2-L (MR) & \texttt{ATOMIC} & $59.2(\pm 0.3)$ & $48.0(\pm 0.9)$ & $67.5(\pm 0.7)$ & $53.5(\pm 0.4)$ & $54.7(\pm 0.6)$\\ 
      GPT2-L (MR) & \texttt{CWWV} & $58.3(\pm 0.4)$ & $46.2(\pm 1.0)$ & $68.6(\pm 0.7)$ & $48.0(\pm 0.7)$ & $52.8(\pm 0.9)$\\
      GPT2-L (MR) & \texttt{CSKG} & $59.0(\pm 0.5)$ & $48.6(\pm 1.0)$ & $68.6(\pm 0.9)$ & $53.3(\pm 0.5)$ & $54.1(\pm 0.5)$\\
      RoBERTa-L (MR) & \texttt{ATOMIC} & $\bf 70.8(\pm 1.2)$  &  $64.2(\pm 0.7)$ &  $72.1(\pm 0.5)$ & $63.1(\pm 1.5)$ & $59.6(\pm 0.3)$\\
      RoBERTa-L (MR) & \texttt{CWWV} & $70.0(\pm 0.3)$ &  $\bf 67.9(\pm 0.8)$ & $72.0(\pm 0.7)$  & $54.8(\pm 1.2)$ & $59.4(\pm 0.5)$ \\
      RoBERTa-L (MR) & \texttt{CSKG} & $70.5(\pm 0.2)$ & $67.4(\pm 0.8)$ & $\bf 72.4(\pm 0.4)$ & $\bf 63.2(\pm 0.7)$ & $\bf 60.9(\pm 0.8)$ \\
      \midrule
      \it RoBERTa-L (supervised) & - & 85.6  & 78.5 & 79.2 & 76.6 & 79.3 \\
      \midrule
      \it Human & - & 91.4 & 88.9 & 94.9 & 86.9 & 94.1 \\
    \bottomrule
    \end{tabular}
  \end{center}
\end{table*}


\subsection{Tasks}
\cut{\filip{I wouldn’t put parts of the framework after ‘tasks’}}
We select commonsense tasks based on two criteria. Firstly, we strive to cover a diverse set of tasks, both in terms of their format (question answering, pronoun resolution, natural language inference), as well as their type of knowledge (e.g., social or physical knowledge). Secondly, we prefer larger task datasets that are manually constructed. For this reason, we do not include datasets like COPA~\cite{gordon-etal-2012-semeval}, or HellaSwag~\cite{zellers-etal-2019-hellaswag}. We opt for the following five task datasets:


\subsubsection{1. Abductive NLI (aNLI)}~\cite{bhagavatula2019abductive} is posed as a natural language inference task. Given the beginning and the ending of a story, the task is to choose the more plausible hypothesis out of two options. The dataset consists of nearly 170k entries.

\subsubsection{2. CommonsenseQA (CSQA)}~\cite{talmor-etal-2019-commonsenseqa} evaluates a broad range of common sense aspects. %focuses broadly on daily commonsense. 
Each entry contains a question and 5 answer candidates. The questions are crowdsourced based on a subgraph from \texttt{ConceptNet}. The answer candidates combine \texttt{ConceptNet} nodes with additional crowdsourced distractors. 

\subsubsection{3. PhysicalIQA (PIQA)}~\cite{Bisk2020} is a two-choice question answering dataset which focuses on physical reasoning. Given a question, the system (or human) is asked to pick the more plausible out of two possible continuations.

\subsubsection{4. SocialIQA (SIQA)}~\cite{sap-etal-2019-social} is a question-answering dataset which requires reasoning about social interactions. Each entry contains a context, a question, and 3 answer candidates. The context is derived from the \texttt{ATOMIC} knowledge graph, the questions are generated based on nine templates (corresponding to the relations in \texttt{ATOMIC}), and the answers are crowdsourced. 


%\subsubsection{COPA}~\cite{gordon-etal-2012-semeval}\filip{remove this?} tests causal reasoning through manually created questions. Each entry contains a premise and 2 candidate answers. The questions are divided into \textit{cause} and \textit{effect} type. 

% \subsubsection{HellaSwag}~\cite{zellers-etal-2019-hellaswag} asks models to select a reasonable continuation in a video sequence or a procedural advice. %, this task aims to test models' commonsense inference ability. 
% Each entry contains a context and 4 candidates continuations. The context and the correct continuation are extracted from ActivityNet and WikiHow, whereas the distractors are first generated by GPT and then adversarially filtered using BERT. 


\subsubsection{5. WinoGrande (WG)}~\cite{sakaguchi2019winogrande} contains 44 thousand pronoun resolution problems. Each entry consists of a context description with an emphasized pronoun, and two options are offered as its possible references.% of this pronoun. 



\section{Experimental Setup}
\subsection{Baselines}
We compare our results with the following baselines. \textit{Majority} answers each question with the most frequent option in the entire dataset. \textit{`Vanilla' versions of the language models} are used in order to understand the impact of further tuning. Here we directly uses the LMs to score the QA pairs without any finetuning. We also show the results of other unsupervised systems that leverage KGs: \textit{Self-talk}, \textit{COMET-}\textit{DynaGen}, and \textit{SMLM}. To indicate the upper bound of this work, we include results of a supervised fine-tuned RoBERTa system and of human evaluation.%\filip{also gpt-2?}


\subsection{Implementation}
For the LM baselines, we directly load the weights from the Transformers library~\cite{Wolf2019HuggingFacesTS} and evaluate on the downstream tasks. The finetuned LMs are trained for a single epoch on our synthetic QA set. For Adv-filter, \cut{In the AFLite condition, }we train the models for 5 epochs to compensate for less training data. We use our synthetic dev set to select the best model.\cut{ checkpoints.} We describe other hyper-parameters used and computing infrastructure in the appendix.


\subsection{Hypotheses}
\label{ssec:hypotheses}

Based on individual prior findings and understanding of different components of our framework, we put forward a set of hypotheses which will be validated in our experiments:%\filip{lets add a sentence for each hypothesis on prior work that investigated it (partially)}

\begin{enumerate}[label=H\arabic*]
    \item \textit{RoBERTa would have better performance than GPT-2.} This is in line with prior findings that RoBERTa has the advantage of bi-directional context~\cite{Zhou2020EvaluatingCI}.
    \item \textit{Pre-training a language model with artificially created question-answer sets enhances zero-shot performance.} This is also supported in previous study about unsupervised QA \cite{li-etal-2020-harvesting}
    %This is an implicit assumption in prior data augmentation work~\cite{kocijan-etal-2019-surprisingly}.
    \item \textit{The impact of more knowledge depends on the alignment between KGs and the task}, partial evidence for which is provided by~\cite{ma-etal-2019-towards,mitra2019exploring}.
    \item \textit{Adding diverse knowledge (from different KGs) improves performance}. This is the initial motivation behind the creation of \texttt{CSKG}~\cite{ilievski2020consolidating}, but has not been investigated in detail.
    \item \textit{When selecting negative samples for a question, it helps to use an adversarial strategy that ensures the question is not trivial for a language model.} H5 is inspired by adversarial filtering, which has not been investigated in detail for automatically-generated questions and across KGs.
    \item \textit{Preserving the task structure when generating synthetic data leads to better accuracy.}
    This is implicitly assumed in prior data augmentation work \cite{kocijan-etal-2019-surprisingly}.
    %Marginal ranking loss yields better performance compared to masked language modeling loss.}%~\cite{tamborrino-etal-2020-pre}.
    %The marginal ranking loss has been proposed by~\citet{tamborrino-etal-2020-pre}, which provides partial support for H6.
    \item \textit{The automatically created questions are notably easier for humans than they are for machines} - a general assumption made by commonsense task creators and typically correct for any existing, human-generated benchmark.
\end{enumerate}


\begin{table*}[]
    \centering
    \caption{Comparison of different QA generation strategies.}
    \begin{tabular}{lcccccc}
         \toprule
         \bf RoBERTa-L & \bf Strategy & \bf aNLI  & \bf CSQA & \bf PIQA & \bf SIQA & \bf WG \\
      \midrule
       \hspace{1em} +\texttt{ATOMIC} & Random & $\bf 70.8(\pm 1.2)$  &  $\bf 64.2(\pm 0.7)$ &  $72.1(\pm 0.5)$ & $\bf 63.1(\pm 1.5)$ & $59.6(\pm 0.3)$\\
       \hspace{1em}  +\texttt{ATOMIC} & Adv-answer & $70.4(\pm 0.8)$ & $62.3 (\pm 0.9)$ & $\bf 72.6(\pm 1.8)$ & $61.6(\pm 0.3)$ & $60.5(\pm 0.5)$  \\
       \hspace{1em} +\texttt{ATOMIC} & Adv-question & $70.8(\pm 0.6)$ & $55.6(\pm 0.9)$ & $70.6(\pm 0.8)$ & $51.6(\pm 0.8)$ & $58.5(\pm 0.3)$ \\
        \hspace{1em} +\texttt{ATOMIC} & Adv-filter & $68.6(\pm 1.8)$ & $46.4(\pm 1.5)$ & $67.9(\pm 1.1)$ & $51.8(\pm 1.2)$ & $\bf 60.8(\pm 0.6)$ \\
        \midrule
       \hspace{1em}  +\texttt{CWWV} & Random & $\bf 70.0(\pm 0.3)$ &  $ 67.9(\pm 0.8)$ & $72.0(\pm 0.7)$  & $\bf 54.8(\pm 1.2)$ & $59.4(\pm 0.5)$ \\
       \hspace{1em} +\texttt{CWWV} & Adv-answer & $69.5(\pm 1.1)$ & $\bf 68.5(\pm 0.8)$ & $\bf 72.7(\pm 0.3)$ & $53.8(\pm 0.6)$ & $\bf 60.7(\pm 0.7)$ \\
       \hspace{1em} +\texttt{CWWV} & Adv-question & $68.3(\pm 2.3)$ & $60.9(\pm 2.3)$ & $69.6(\pm 0.6)$ & $47.0(\pm 2.0)$ & $59.0(\pm 1.4)$ \\
       \hspace{1em} +\texttt{CWWV} & Adv-filter & $69.7(\pm 0.7)$ & $64.7(\pm 2.3)$ & $72.0(\pm 1.3)$ & $50.1(\pm 1.0)$ & $59.4(\pm 1.4)$ \\
      \bottomrule
    \end{tabular}
    \label{tab:generation}
\end{table*}

==> Zero-shot Question Answering using Knowledge Bases/4-results.tex <==






\section{Results}
We evaluate various combinations of: knowledge sources, question generation strategies, LMs, training regimes, and tasks. We use accuracy as a metric. All our experiments are performed in a zero-shot setting, i.e., the models do not leverage the official training data of the task. We report results on the dev sets of these tasks, as the official test sets are not publicly available. We note that, since we did not use the tasks' dev sets for hyperparameter tuning or checkpoint selection, the dev sets can be used effectively as test sets. 

\subsection{Main Results}
Table 2 shows that GPT-2 and RoBERTa outperform the majority baseline by a large margin on all tasks, indicating that the LMs have already learned relevant knowledge during pretraining. Despite being a smaller model, RoBERTa outperforms GPT-2 on 4 out of 5 tasks without pretraining, and on all tasks when pretraining over different synthetic QA sets. This shows the advantage of leveraging bi-directional context, and confirms our hypothesis H1. As expected (H2), training RoBERTa on our \texttt{ATOMIC} or \texttt{CWWV} synthetic sets brings notable performance gain on all 5 tasks. We observe that models trained on \texttt{ATOMIC} sets have a large advantage on SIQA compare to models trained on \texttt{CWWV}, while \texttt{CWWV} brings advantage on the CSQA task. This is not surprising as these two tasks are derived from \texttt{ConceptNet} and \texttt{ATOMIC}, respectively. The difference between \texttt{ATOMIC} and \texttt{CWWV} on the remaining three tasks is relatively small. This supports our hypothesis H3: knowledge alignment is crucial for obtaining better performance.

Training on the combined question set (\texttt{CSKG}) is mostly able to retain the best of its both partitions. Training on \texttt{CSKG} leads to best performance on three out of five tasks, showing that a global commonsense resource is able to bring consistent gain across different tasks. This supports our hypothesis H4: adding more diverse knowledge is beneficial for language models. Finally, even with this knowledge, we recognize that there is still a large gap between our model's accuracy and that of the supervised RoBERTa model. 


\cut{\subsection{Few-shot Evaluation}
Following previous work, we also experimented our model in few-shot condition. Here we randomly sampled 2400 examples in the training set (~8\% of training set) and continue trained our model. The results are shown in table \ref{tab:few-shot}. Our model pretrained on the synthetic data is able to outperform the baseline models and previous approach, showing that our proposed approach could be useful for the low-resource setting as well. Moreover, it is worth noting that our model in few-shot setting is able to achieve similar performance to that of the RoBERTa model using the entire training set. }




\subsection{Comparison of QA Generation Strategies}

%, making it harder for the model to distinguish the answer candidates. 

Table~\ref{tab:generation} shows the results with different sampling strategies, thus addressing H5. The best performing adversarial algorithm, \textit{Adv-answer}, yields comparable accuracy to the \textit{random} strategy, revealing that distractors sampled with a more sophisticated strategy are not necessarily more informative for the LMs. \textit{Adv-question} and \textit{Adv-filter} typically lead to declines in accuracy. Considering \textit{Adv-question}, this could be due to the similarity of the distractors to the question, which might guide the model to learn to pick the most dissimilar candidate as the correct answer, which is an artifact of our question generation and cannot be expected to work well for downstream tasks. \cut{Finally, the results for \textit{Adv-filter} dropped significantly on some tasks. }
Our manual inspection of the remaining questions prefered by \textit{Adv-filter} indicates that many questions are unfair, as some distractors are also correct answers, which is a consequence of the incompleteness of the KGs. \cut{, even with our strict rule-based filter, the distractor pool may still contain some unfair distractors.} 
Adv-filter prioritizes these questions as they are ``difficult'' for LMs, however, training on them might teach the LM incorrect knowledge and harm downstream accuracy. %This finding informs H5: \textit{random} sampling, although being the simplest strategy, performs comparably to the best adversarial strategy. % might be the best option to adopt.


\subsection{Comparison of Training Regimes}
Table~\ref{tab:regimes} presents results with two different training regimes. In comparison to the baseline without additional training, MLM training on \texttt{ATOMIC} only improves on the SIQA task, and harms on the rest. With \texttt{CWWV}, it brings large gain on CSQA and small improvements on SIQA and WG. At the same time, marginal ranking training on either question set consistently outperforms MLM training by a large margin, suggesting that preserving the task structure is beneficial in addition to the question content and validating H6.




\subsection{Difficulty of the Synthetic QA Sets}
Ideally, the generated question-answer pairs should be challenging for the models but easy for humans to solve (H7).
%We hypothesize that a good commonsense question is easier for humans than for language models, allowing them to learn useful information which is obvious for humans (H7).
Here, we probe this hypothesis by assessing the difficulty of our synthetic QA sets both by humans and `vanilla' LMs. %Thus we evaluate the GPT2 and RoBERTa baseline models on our synthetic QA sets and conduct human evaluation. 
We evaluated both models on the dev sets of our synthetic data. 
For human evaluation, we randomly sample 50 questions from \texttt{ATOMIC} and 50 questions from \texttt{CWWV}. A total of five researchers were asked to first \textit{provide the correct answer}, then \textit{rate the question difficulty}. For the latter, the annotator chose between easy, moderate, hard, or non-sensical - as a guideline, nonsensical questions have unfair distractors and cannot be easily understood. Following this procedure, we obtained three judgments for each question. 

The inter-annotator agreement on selecting the correct answer is 0.62 using Fleiss Kappa score, which is substantial agreement. The Kripendorf alpha \cite{krippendorff04} for rating question difficulty is 0.35, which is fair agreement. The results of the baseline LMs and human performance (Table~\ref{tab:difficulty}) show that the \texttt{ATOMIC} subset presents a harder challenge for both models, as well as for humans. Overall, the results support our hypothesis H7: the synthetic questions are relatively easy for humans to solve and much harder for models. However, the annotation pointed to several directions for improving the synthetic QA sets. A number of questions generated from \texttt{ATOMIC} are ungrammatical, which makes them harder to understand, while some questions from \texttt{CWWV} were rated as unfair. For example, all answer options for the question \textit{A person can} are valid: (a) \textit{cost several thousand dollars} (b) \textit{expressing boredom} (c) \textit{check snow level}. As discussed earlier, this is due to the incompleteness of our KGs, and the current lack of understanding on how to generate fair, yet informative, distractors. 

\begin{table}
  \begin{center}
    \caption{Comparison between MLM and MR training.}
    \label{tab:regimes}
    \begin{tabular}{@{}ll@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{\hspace{7pt}}c@{}} 
     \toprule
      RoBERTa-L & Train & aNLI & CSQA & PIQA & SIQA & WG\\
        \midrule 
       baseline & - & 65.5  & 45.0 &  67.6 & 47.3 & 57.5 \\
      + \texttt{ATOMIC} & MLM & 62.9 & 43.8 & 65.8 & 53.9 & 55.5 \\
      + \texttt{ATOMIC} & MR & 70.8 & 64.2 & 72.1 & 63.1 & 59.6 \\
      + \texttt{CWWV} & MLM & 65.3 & 57.3 & 67.2 & 49.3 & 59.4 \\
      + \texttt{CWWV} & MR & 70.0 & 67.9 & 72.0 & 54.8 & 59.4 \\
    \bottomrule
    \end{tabular}
  \end{center}
\end{table}






==> Zero-shot Question Answering using Knowledge Bases/5-discussion.tex <==
\section{Discussion}

\subsection{Towards a Commonsense Service}

The overarching pursuit of this paper is to understand whether generating artificial QA sets with KGs improves the zero-shot QA performance of LMs. We observe a consistent leap in accuracy across tasks, LMs, knowledge sources, and question generation strategies. While these accuracies are notably below supervised LM accuracies, they might further improve by architectural improvements of the LMs, knowledge sources with wider coverage and stronger semantics, and well-tuned scoring functions.\footnote{For example, scoring sequences of tokens by a language model might improve the performance of LMs \cite{tamborrino-etal-2020-pre}.} 
In addition, despite its complexity and diversity, commonsense knowledge (unlike knowledge on entities and events, which changes rapidly) is largely static and evolves slowly over time, thus making the dataset-specific finetuning unnecessary in theory.
A natural question arises: can we build a sufficiently reliable, general commonsense service, by pretraining a LM on a rich set of questions covering a wide spectrum of knowledge types? 






\subsection{Impact of Knowledge}

In general, we observed that using knowledge from a wider set of sources is beneficial. However, on \anli~and \csqa, the best accuracy was obtained with a subset of all questions. This could be due to the kinds of knowledge covered: 
\begin{enumerate*}
\item \anli~focuses on expectations of agents and events, for which \texttt{ATOMIC} is directly useful, whereas the other KGs might be delusive;
\item \csqa~mostly requires knowledge about properties of objects (e.g., function or appearance) which is the focus of \texttt{ConceptNet},~\texttt{Wikidata}, and \texttt{VisualGenome}, but not of \texttt{ATOMIC}.
\end{enumerate*}
This indicates a tension between H3 and H4: while more knowledge often helps, it might not be the case when the task and the knowledge are not well-aligned. Our current understanding of the dimensions of commonsense knowledge in knowledge sources and benchmarks is limited, and would benefit from further study.



\begin{table}
  \begin{center}
    \caption{LM and human accuracy on our synthetic QA sets.}
    \label{tab:difficulty}
    \begin{tabular}{lcc} 
     \toprule
      Model & ATOMIC & CWWV\\
      \midrule
      GPT2-L & 43.2 & 69.5 \\
      RoBERTa-L & 45.9 & 64.5 \\
      Human & 78.0 & 80.7\\
      \bottomrule
    \end{tabular}
  \end{center}
\end{table}


\subsection{Generating Fair and Informative Questions}

Alternatively, this result may be explained \cut{An alternative explanation for this result is indicated }by our human evaluation: not all automatically generated questions are fair and a subset has more than one correct answer, as a direct consequence of the inherent incompleteness of KGs. % according to our manual inspection.
Besides being a disadvantage of automatic question generation, this finding points to a more substantial challenge: generating fair and informative multiple-choice questions is not yet well-understood. \cut{In an independent annotation study, the authors found that out of 200 questions from the \csqa~dataset that were answered incorrectly by  HyKAS~\cite{ma-etal-2019-towards}, \filip{number here + anonymize system} had more than one correct answer according to human annotators.} Adversarial strategies yield more plausible candidates than random sampling, making the task less fair; yet, fully relying on random sampling would generate distractors that are trivially discernible from the correct option. Balancing between fairness and informativeness, thus, is essential for multiple-choice question generation. Our empirical evidence suggests that it could be achieved by a mixed approach, where part of distractors is generated randomly, and part by adopting suitable adversarial strategies.\footnote{Question formulation is another challenge. Template-based questions may be trivially easy for LMs to solve, as discussed in \url{https://cs.nyu.edu/faculty/davise/papers/CYCQns.html}.}


 %On a different note, 


\cut{\subsection{Scoring function}
While our scoring function already achieves strong performance across different tasks, we recognize that there are other scoring functions that may further improve the scores. For example, \cite{tamborrino-etal-2020-pre} showed that for masked language models, one can mask our N consecutive tokens at a time and to compute the score for sequences. The combination of scores computed when N=1,2,3... works better than N=1. However, such method also implies larger computational cost in both pretraining and evaluation stage. Since our main goal is not to achieve the SOTA performance, we leave the exploration of better scoring function for future work. \filip{this is useful but perhaps we can turn it into 'Limitations of the Framework' and discuss other things that we havent done yet}}



==> Zero-shot Question Answering using Knowledge Bases/6-conclusion.tex <==
\section{Conclusions}

While zero-shot QA is gaining focus, no study so far has investigated systematically the dependency between the task, the technique, and any additional knowledge used. To address this gap, this paper proposed a framework for zero-shot QA by pretraining LMs on artificial data created based on KGs. We studied the interplay between five knowledge sources, four data generation strategies, two LMs, two training regimes, and five tasks. We put forward seven hypotheses, which guided our experiments. We observed that language models benefit from pretraining on artificially created QA sets. Similar to prior work, we observed that the best performance is obtained by the RoBERTa model. Furthermore, combining knowledge sources leads to best performance, indicating that diverse relevant knowledge is desired for pretraining. However, this is conditioned on a good alignment between knowledge and the task. The training regime had a role too: marginal ranking is superior to vanilla language modeling, as it preserved better the structure of the task. Our analysis and human evaluation indicated that the generated questions were typically easier for humans than for language models, which is appropriate for commonsense questions.

Yet, the human evaluation revealed that a notable portion of the questions is nonsensical or difficult, hinting that automatically generating high-quality, informative commonsense questions is non-trivial and should be revised in subsequent work. Future work should also investigate the impact of this approach on knowledge injection systems~\cite{ma-etal-2019-towards} and graph relational networks~\cite{lin-etal-2019-kagnet}. It should also consider: (1) other, less structured knowledge sources, like WikiHow; (2) different distractor sampling strategies, e.g., based on iterative sampling \cite{niu2020self}; and (3) additional LM scoring functions, e.g., based on scoring sequences of tokens~\cite{tamborrino-etal-2020-pre}.

==> Zero-shot Question Answering using Knowledge Bases/old-1-intro.tex <==
\section{Introduction}

Quick statement on commonsense reasoning, in general, specification of their downsides, then a (very) quick transition to neural methods...

Hypothesis: structure in the background context (e.g., for pre-training) plays a huge part in performance on social-interaction QA tasks. Further, we said in (Ma et al., 2019): \textit{external knowledge is only helpful when there is alignment between questions and knowledge-base types.}

Observation: 
1. pretraining on data generated from Conceptnet didn't work as well as pretraining on OMCS directly; information loss, due to structural differences? (argument made from previous work) (here they simply used simple templates to convert ConceptNet triples to sentences)\\
2. Another previous work pretrain the model on OMCS and use ConceptNet relations to guide word/span masking and distractor selection, showing that this is better than using OMCS. \\

Approach: generate a separate view of the background context in the form of a QA dataset

Experiment: Because we are attempting to study how structure of the background context affects models' inductive capabilities, we perform experiments under zero-shot condition (preferably, on more than one task).

Initial motivation: \\
1. OCN component is not pretrained for regular MLM pre-training task \\
2. By reducing the answer space from entire tail set of ATOMIC to only a few, we make the pretraining task easier for model to learn (why would this be better? where is the training signal coming from, that biases the model to prefer the subset over the entire tail set?)\\
3. Why is the structure important? (we want to make the synthetic data look more like the task we care about, yes, but why is that important -- e.g., from a representation learning perspective?)

Other experiments we want to consider: 
1. Include entire CSKG for Synthetic data generation / pretraining, depends on the results, we then decide whether to include it or not 
3. Include other tasks, such as CommonsenseQA in the zero-shot evaluation, and we would want to compare with RoBERTa and GPT-2 zero-shot baseline 

Another thought: In socialIQa paper, they experimented with COPA and WSC to show that training on SocialIQa help transfer knowledge to these 2 tasks. However, for these small tasks, they usually use dev set for training, which seems a bit weak. Maybe we can show that our way of doing things can truly achieve zero-shot on these tasks? 

In self-talk paper, they mentioned "We also experimented with combining the clarifications from all the knowledge sources, which didn’t prove beneficial except for MCTACO" and
"that when the datasets were created using a knowledge source clarifications from that resource are considered correct. We also note that somewhat surprisingly, relatively few ConceptNet clarifications were considered correct, despite limiting the relation paths up to 2 edges."

==> Zero-shot Question Answering using Knowledge Bases/old-2-relatedwork.tex <==
\section{Related Work}

\subsection{Neural Commonsense Reasoning}

\begin{itemize}
    \item General background on using neural models for commonsense
    \item Some approaches just rely on using language models (e.g., without any external knowledge resources and/or without any \textit{task-specific} commonsense injection mechanisms)
    \item MLM pre-training, which may not be best-suited for CS MC QA tasks
\end{itemize} 

\subsection{Knowledge-injection Methods}
Numerous research have studied ways of injecting external knowledge into neural models in recent years. In terms of knowledge resources, several popular knowledge bases has been studied extensively such as ConceptNet \cite{10.5555/3298023.3298212}, WordNet \cite{10.1145/219717.219748}, and ATOMIC \cite{DBLP:conf/aaai/SapBABLRRSC19}. Regarding the neural models, the pretrained language models has become the default choice for many tasks due to their strong performance, including BERT \cite{devlin-etal-2019-bert}, RoBERTa \cite{Liu2019RoBERTaAR}, and GPT \cite{radford2019language}. For knowledge injection methods, one line of work typically extract a subgraph for each question-answer pair, then the sub-graph is encoded and injected into the context/question encoding via attention mechanism \cite{bauer-etal-2018-commonsense,lin-etal-2019-kagnet,ma-etal-2019-towards} or through an auxiliary training objective \cite{10.1145/3357384.3358165}. In other cases, the encoded knowledge sub-graph is directly used to score answer candidates \cite{10.1007/978-3-030-32233-5_2}. (FI: I think KagNet (Lin et al., 2019) and MultiGRN (Lin et al., 2020) also fall in the graph category.)  Another line of work propose to incorporate entire knowledge bases in the pretraining phrase by introducing additional modeling objectives, therefore equip the language models with structured knowledge \cite{peters-etal-2019-knowledge,levine-etal-2020-sensebert,Liu2020KBERTEL,zhang-etal-2019-ernie,talmor2020teaching}. (FI: I think the par could be shortened in the beginning; but we should finish by saying how we compare to this work)

\subsection{Zero-shot Question Answering}
Unsupervised methods have been explored in previous works to solve question answering tasks \cite{li-etal-2020-harvesting}. (FI: what is this citation for?) 
Assuming low availability of training data, the Self-training Method \cite{niu2020self} enhances the small set of golden labels with noisy evidence labels, and uses the pseudo evidence predictions as extra supervision in the next iteration.
Several previous work have also attempted to solve commonsense reasoning tasks in a zero-shot fashion. \cite{Bosselut2019DynamicKG} proposed to use COMET, a generative model trained on commonsense knowledge graphs, to generate knowledge statement for each context. Then the COMET model is used again to compute scores for each answer candidate based on the context, question and generated knowledge. \cite{Shwartz2020UnsupervisedCQ} proposed a Self-Talk model, where a set of clarification questions are first generated using the pretrained-LM conditioned on template prefix, and then the generated questions are used to elicit knowledge from another pretrained-LM. Then the elicited knowledge is used jointly with original context and question to score each answer candidate. The work from \cite{Banerjee2020SelfsupervisedKT} is the most similar to ours, where they proposed to pretrain the LM solely based on knowledge graphs. They trained 3 mapping functions to recover the third element in the knowledge triple given the other 2. Then these functions are used jointly to compute the distance for each answer candidate. (FI: we need closure to this par too; how we compare to this work)

==> old-1-intro.tex <==
\section{Introduction}

Quick statement on commonsense reasoning, in general, specification of their downsides, then a (very) quick transition to neural methods...

Hypothesis: structure in the background context (e.g., for pre-training) plays a huge part in performance on social-interaction QA tasks. Further, we said in (Ma et al., 2019): \textit{external knowledge is only helpful when there is alignment between questions and knowledge-base types.}

Observation: 
1. pretraining on data generated from Conceptnet didn't work as well as pretraining on OMCS directly; information loss, due to structural differences? (argument made from previous work) (here they simply used simple templates to convert ConceptNet triples to sentences)\\
2. Another previous work pretrain the model on OMCS and use ConceptNet relations to guide word/span masking and distractor selection, showing that this is better than using OMCS. \\

Approach: generate a separate view of the background context in the form of a QA dataset

Experiment: Because we are attempting to study how structure of the background context affects models' inductive capabilities, we perform experiments under zero-shot condition (preferably, on more than one task).

Initial motivation: \\
1. OCN component is not pretrained for regular MLM pre-training task \\
2. By reducing the answer space from entire tail set of ATOMIC to only a few, we make the pretraining task easier for model to learn (why would this be better? where is the training signal coming from, that biases the model to prefer the subset over the entire tail set?)\\
3. Why is the structure important? (we want to make the synthetic data look more like the task we care about, yes, but why is that important -- e.g., from a representation learning perspective?)

Other experiments we want to consider: 
1. Include entire CSKG for Synthetic data generation / pretraining, depends on the results, we then decide whether to include it or not 
3. Include other tasks, such as CommonsenseQA in the zero-shot evaluation, and we would want to compare with RoBERTa and GPT-2 zero-shot baseline 

Another thought: In socialIQa paper, they experimented with COPA and WSC to show that training on SocialIQa help transfer knowledge to these 2 tasks. However, for these small tasks, they usually use dev set for training, which seems a bit weak. Maybe we can show that our way of doing things can truly achieve zero-shot on these tasks? 

In self-talk paper, they mentioned "We also experimented with combining the clarifications from all the knowledge sources, which didn’t prove beneficial except for MCTACO" and
"that when the datasets were created using a knowledge source clarifications from that resource are considered correct. We also note that somewhat surprisingly, relatively few ConceptNet clarifications were considered correct, despite limiting the relation paths up to 2 edges."

==> old-2-relatedwork.tex <==
\section{Related Work}

\subsection{Neural Commonsense Reasoning}

\begin{itemize}
    \item General background on using neural models for commonsense
    \item Some approaches just rely on using language models (e.g., without any external knowledge resources and/or without any \textit{task-specific} commonsense injection mechanisms)
    \item MLM pre-training, which may not be best-suited for CS MC QA tasks
\end{itemize} 

\subsection{Knowledge-injection Methods}
Numerous research have studied ways of injecting external knowledge into neural models in recent years. In terms of knowledge resources, several popular knowledge bases has been studied extensively such as ConceptNet \cite{10.5555/3298023.3298212}, WordNet \cite{10.1145/219717.219748}, and ATOMIC \cite{DBLP:conf/aaai/SapBABLRRSC19}. Regarding the neural models, the pretrained language models has become the default choice for many tasks due to their strong performance, including BERT \cite{devlin-etal-2019-bert}, RoBERTa \cite{Liu2019RoBERTaAR}, and GPT \cite{radford2019language}. For knowledge injection methods, one line of work typically extract a subgraph for each question-answer pair, then the sub-graph is encoded and injected into the context/question encoding via attention mechanism \cite{bauer-etal-2018-commonsense,lin-etal-2019-kagnet,ma-etal-2019-towards} or through an auxiliary training objective \cite{10.1145/3357384.3358165}. In other cases, the encoded knowledge sub-graph is directly used to score answer candidates \cite{10.1007/978-3-030-32233-5_2}. (FI: I think KagNet (Lin et al., 2019) and MultiGRN (Lin et al., 2020) also fall in the graph category.)  Another line of work propose to incorporate entire knowledge bases in the pretraining phrase by introducing additional modeling objectives, therefore equip the language models with structured knowledge \cite{peters-etal-2019-knowledge,levine-etal-2020-sensebert,Liu2020KBERTEL,zhang-etal-2019-ernie,talmor2020teaching}. (FI: I think the par could be shortened in the beginning; but we should finish by saying how we compare to this work)

\subsection{Zero-shot Question Answering}
Unsupervised methods have been explored in previous works to solve question answering tasks \cite{li-etal-2020-harvesting}. (FI: what is this citation for?) 
Assuming low availability of training data, the Self-training Method \cite{niu2020self} enhances the small set of golden labels with noisy evidence labels, and uses the pseudo evidence predictions as extra supervision in the next iteration.
Several previous work have also attempted to solve commonsense reasoning tasks in a zero-shot fashion. \cite{Bosselut2019DynamicKG} proposed to use COMET, a generative model trained on commonsense knowledge graphs, to generate knowledge statement for each context. Then the COMET model is used again to compute scores for each answer candidate based on the context, question and generated knowledge. \cite{Shwartz2020UnsupervisedCQ} proposed a Self-Talk model, where a set of clarification questions are first generated using the pretrained-LM conditioned on template prefix, and then the generated questions are used to elicit knowledge from another pretrained-LM. Then the elicited knowledge is used jointly with original context and question to score each answer candidate. The work from \cite{Banerjee2020SelfsupervisedKT} is the most similar to ours, where they proposed to pretrain the LM solely based on knowledge graphs. They trained 3 mapping functions to recover the third element in the knowledge triple given the other 2. Then these functions are used jointly to compute the distance for each answer candidate. (FI: we need closure to this par too; how we compare to this work)
